Complex Spin: The Missing Zeroes and Newton's Dark Magic

Conformal Regge theory predicts the existence of analytically continued CFT data for complex spin. How could this work when there are so many more operators with large spin compared to small spin? Using planar N=4 SYM as a testground we find a simple physical picture. Operators do organize themselves into analytic families but the continuation of the higher families have zeroes in their structure OPE constants for lower integer spins. They thus decouple. Newton's interpolation series technique is perfectly suited to this physical problem and will allow us to explore the right complex spin half-plane.

==> biblioold.tex <==
\bibitem{hexagons}
B.~Basso, S.~Komatsu and P.~Vieira,
``Structure Constants and Integrable Bootstrap in Planar N=4 SYM Theory,''
[arXiv:1505.06745].

\bibitem{kolyaQSC}
N.~Gromov, V.~Kazakov, S.~Leurent and D.~Volin,
``Quantum Spectral Curve for Planar $\mathcal{N} = 4$ Super-Yang-Mills Theory,''
Phys. Rev. Lett. \textbf{112}, no.1, 011602 (2014)
%doi:10.1103/PhysRevLett.112.011602
[arXiv:1305.1939].
$\bullet$
N.~Gromov, V.~Kazakov, S.~Leurent and D.~Volin,
``Quantum spectral curve for arbitrary state/operator in AdS$_{5}$/CFT$_{4}$,''
JHEP \textbf{09}, 187 (2015)
%doi:10.1007/JHEP09(2015)187
[arXiv:1405.4857].

\bibitem{wrappingthreeBGKV}
B.~Basso, V.~Goncalves, S.~Komatsu and P.~Vieira,
``Gluing Hexagons at Three Loops,''
Nucl. Phys. B \textbf{907}, 695-716 (2016)
%doi:10.1016/j.nuclphysb.2016.04.020
[arXiv:1510.01683]. 

\bibitem{wrappingshota}
B.~Basso, V.~Goncalves and S.~Komatsu,
``Structure constants at wrapping order,''
JHEP \textbf{05}, 124 (2017)
%doi:10.1007/JHEP05(2017)124
[arXiv:1702.02154].

\bibitem{wrappingthreeES} B.~Eden and A.~Sfondrini,
``Three-point functions in ${\cal N}=4$ SYM: the hexagon proposal at three loops,''
JHEP \textbf{02}, 165 (2016)
%doi:10.1007/JHEP02(2016)165
[arXiv:1510.01242]

\bibitem{tailoring0}
R.~Roiban and A.~Volovich,
``Yang-Mills correlation functions from integrable spin chains,''
JHEP \textbf{09} (2004), 032
%doi:10.1088/1126-6708/2004/09/032
[arXiv:hep-th/0407140].

%\cite{Vieira:2013wya}
\bibitem{Wang}
P.~Vieira and T.~Wang,
``Tailoring Non-Compact Spin Chains,''
JHEP \textbf{10} (2014), 035
%doi:10.1007/JHEP10(2014)035
[arXiv:1311.6404].
%38 citations counted in INSPIRE as of 06 Sep 2022

\bibitem{tailoring}
J.~Escobedo, N.~Gromov, A.~Sever and P.~Vieira,
``Tailoring Three-Point Functions and Integrability,''
JHEP \textbf{09}, 028 (2011)
%doi:10.1007/JHEP09(2011)028
[arXiv:1012.2475].

%\cite{Derkachov:2002tf}
\bibitem{Derkachov}
S.~E.~Derkachov, G.~P.~Korchemsky and A.~N.~Manashov,
``Separation of variables for the quantum SL(2,R) spin chain,''
JHEP \textbf{07} (2003), 047
%doi:10.1088/1126-6708/2003/07/047
[arXiv:hep-th/0210216].
%72 citations counted in INSPIRE as of 06 Sep 2022

\bibitem{clustering}
Y.~Jiang, S.~Komatsu, I.~Kostov and D.~Serban,
``Clustering and the Three-Point Function,''
J. Phys. A \textbf{49} (2016) no.45, 454003
%doi:10.1088/1751-8113/49/45/454003
[arXiv:1604.03575].
%40 citations counted in INSPIRE as of 06 Sep 2022

\bibitem{kolyasu2}
N.~Gromov, F.~Levkovich-Maslyuk, P.~Ryan and D.~Volin,
``Dual Separated Variables and Scalar Products,''
Phys. Lett. B \textbf{806}, 135494 (2020)
%doi:10.1016/j.physletb.2020.135494
[arXiv:1910.13442]

\bibitem{kolyasl3}
A.~Cavagli\`a, N.~Gromov and F.~Levkovich-Maslyuk,
``Separation of variables and scalar products at any rank,''
JHEP \textbf{09}, 052 (2019)
%doi:10.1007/JHEP09(2019)052
[arXiv:1907.03788].

\bibitem{kolyadeterminant}
N.~Gromov, F.~Levkovich-Maslyuk and P.~Ryan,
``Determinant form of correlators in high rank integrable spin chains via separation of variables,''
JHEP \textbf{05}, 169 (2021)
%doi:10.1007/JHEP05(2021)169
[arXiv:2011.08229]

\bibitem{fishnet}
\"O.~G\"urdo\u{g}an and V.~Kazakov,
``New Integrable 4D Quantum Field Theories from Strongly Deformed Planar $\mathcal N = $ 4 Supersymmetric Yang-Mills Theory,''
Phys. Rev. Lett. \textbf{117} (2016) no.20, 201602
%doi:10.1103/PhysRevLett.117.201602
[arXiv:1512.06704].

\bibitem{kolyafishnet}
A.~Cavagli\`a, N.~Gromov and F.~Levkovich-Maslyuk,
``Separation of variables in AdS/CFT: functional approach for the fishnet CFT,''
JHEP \textbf{06}, 131 (2021)
%doi:10.1007/JHEP06(2021)131
[arXiv:2103.15800].

\bibitem{LOHahn}
L.~D.~Faddeev and G.~P.~Korchemsky,
``High-energy QCD as a completely integrable model,''
Phys. Lett. B \textbf{342} (1995), 311-322
%doi:10.1016/0370-2693(94)01363-H
[arXiv:hep-th/9404173].

\bibitem{NLOHahn}
A.~V.~Kotikov, A.~Rej and S.~Zieme,
``Analytic three-loop Solutions for N=4 SYM Twist Operators,''
Nucl. Phys. B \textbf{813} (2009), 460-483
%doi:10.1016/j.nuclphysb.2008.12.022
[arXiv:0810.0691]. $\bullet$ M.~Beccaria, A.~V.~Belitsky, A.~V.~Kotikov and S.~Zieme,
``Analytic solution of the multiloop Baxter equation,''
Nucl. Phys. B \textbf{827} (2010), 565-606
%doi:10.1016/j.nuclphysb.2009.10.030
[arXiv:0908.0520].

\bibitem{bassobelitsky}
B.~Basso and A.~V.~Belitsky,
``Luescher formula for GKP string,''
Nucl. Phys. B \textbf{860}, 1-86 (2012)
%doi:10.1016/j.nuclphysb.2012.02.011
[arXiv:1108.0999].
%31 citations counted in INSPIRE as of 17 Sep 2022

\bibitem{DO}
F.~A.~Dolan and H.~Osborn,
``Conformal four point functions and the operator product expansion,''
Nucl. Phys. B \textbf{599} (2001), 459-496
[arXiv:hep-th/0011040].


\bibitem{reciprocitypapers}
B.~Basso and G.~P.~Korchemsky,
``Anomalous dimensions of high-spin operators beyond the leading order,''
Nucl. Phys. B \textbf{775}, 1-30 (2007)
%doi:10.1016/j.nuclphysb.2007.03.044
[arXiv:hep-th/0612247]
$\bullet$ 
L.~F.~Alday, A.~Bissi and T.~Lukowski,
``Large spin systematics in CFT,''
JHEP \textbf{11}, 101 (2015)
%doi:10.1007/JHEP11(2015)101
[arXiv:1502.07707] 

\bibitem{morphism}
N.~Gromov and P.~Vieira,
``Tailoring Three-Point Functions and Integrability IV. Theta-morphism,''
JHEP \textbf{04}, 068 (2014)
%doi:10.1007/JHEP04(2014)068
[arXiv:1205.5288].

\bibitem{shotaXXX}
Y.~Kazama, S.~Komatsu and T.~Nishimura,
``A new integral representation for the scalar products of Bethe states for the XXX spin chain,''
JHEP \textbf{09}, 013 (2013)
%doi:10.1007/JHEP09(2013)013
[arXiv:1304.5011].

\bibitem{shotamirror}
Y.~ Jiang, S.~ Komatsu, I.~ Kostov, D.~ Serban,
``The hexagon in the mirror: the three-point function in the SoV representation,''
J.Phys.A \textbf{49} (2016) 17, 174007
[arXiv:hep-th/1506.09088]

\bibitem{bottom}
In this section we assume that $\ell_{23}\geq2$ so that bottom mirror corrections can be neglected \cite{wrappingthreeBGKV}. Otherwise, we expect its inclusion to follow a similar prescription as in the SL(2) case.

\bibitem{transcendentality}
It would be desirable to restore naive trascendentality counting, see also discussion at the end of appendix \ref{rootscharges}. 

\bibitem{transcendentality2} 
There is a fun fact about all the $\pi$'s floating around in the SU(2) result -- see the \textit{anomaly} $\delta_{l,2}$ as well as $\alpha$: they are there simply to cancel $\pi$'s generated from the integrations so that the final result is a rational function of the Bethe roots. From a practical point of view we could drop these $\pi$'s provided we also drop any $\pi$'s generated when picking up residues. At higher loops the structure constants are no longer rational and such games would be dangerous.
\bibitem{betheequationsref}
G.~Arutyunov, S.~Frolov and M.~Staudacher,
``Bethe ansatz for quantum strings,''
JHEP \textbf{10}, 016 (2004)
%doi:10.1088/1126-6708/2004/10/016
[arXiv:hep-th/0406256 [hep-th]].
%556 citations counted in INSPIRE as of 30 Sep 2022
\bibitem{BeisertStaudacher}
N.~Beisert and M.~Staudacher,
``Long-range psu(2,2|4) Bethe Ansatze for gauge theory and strings,''
Nucl. Phys. B \textbf{727} (2005), 1-62
%doi:10.1016/j.nuclphysb.2005.06.038
[arXiv:hep-th/0504190].

\bibitem{giombi}
S.~Giombi, S.~Komatsu and B.~Offertaler,
``Large charges on the Wilson loop in $ \mathcal{N} $ = 4 SYM. Part II. Quantum fluctuations, OPE, and spectral curve,''
JHEP \textbf{08}, 011 (2022)
%doi:10.1007/JHEP08(2022)011
[arXiv:2202.07627].

\bibitem{caetano}
J.~Caetano and S.~Komatsu,
``Functional equations and separation of variables for exact $g$-function,''
JHEP \textbf{09}, 180 (2020)
%doi:10.1007/JHEP09(2020)180
[arXiv:2004.05071].

\bibitem{spinninghexagons}
C.~Bercini, V.~Goncalves, A.~Homrich and P.~Vieira,
``Spinning Hexagons,''
[arXiv:2207.08931].

\bibitem{Bianchi:2019jpy}
M.~S.~Bianchi,
``On structure constants with two spinning twist-two operators,''
JHEP \textbf{04}, 059 (2019)
[arXiv:1901.00679].

\bibitem{ourRecentPapers}
C.~Bercini, V.~Gon\c{c}alves, A.~Homrich and P.~Vieira,
``The Wilson loop \textemdash{} large spin OPE dictionary,''
JHEP \textbf{07}, 079 (2022)
[arXiv:2110.04364].

\bibitem{Bassowrap}
B.~Basso, A.~Georgoudis and A.~K.~Sueiro,
``Structure constants of short operators in planar $\mathcal{N}=4$ SYM theory,''
[arXiv:2207.01315].

\bibitem{tunneling}
N.~Gromov, A.~Sever and P.~Vieira,
``Tailoring Three-Point Functions and Integrability III. Classical Tunneling,''
JHEP \textbf{07}, 044 (2012)
%doi:10.1007/JHEP07(2012)044
[arXiv:1111.2349].

\bibitem{Kostov}
I.~Kostov,
``Semi-classical scalar products in the generalised SU(2) model,''
Springer Proc. Math. Stat. \textbf{111}, 87-103 (2014)
%doi:10.1007/978-4-431-55285-7\_7
[arXiv:1404.0235].
$\bullet$
%\cite{Bettelheim:2014gma}
E.~Bettelheim and I.~Kostov,
``Semi-classical analysis of the inner product of Bethe states,''
J. Phys. A \textbf{47}, 245401 (2014)
%doi:10.1088/1751-8113/47/24/245401
[arXiv:1403.0358].

\bibitem{shotastrong}
Y.~Kazama and S.~Komatsu,
``Three-point functions in the SU(2) sector at strong coupling,''
JHEP \textbf{03}, 052 (2014)
%doi:10.1007/JHEP03(2014)052
[arXiv:1312.3727].

\bibitem{BassoDeLiang}
B.~Basso and D.~L.~Zhong,
``Three-point functions at strong coupling in the BMN limit,''
JHEP \textbf{04}, 076 (2020)
%doi:10.1007/JHEP04(2020)076
[arXiv:1907.01534].
%10 citations counted in INSPIRE as of 23 Sep 2022

\bibitem{WIPwithBen}
B.~Basso, C.~Bercini, A.~Homrich, P.~Vieira,
Work in Progress

\bibitem{classicalPaper1}
L.~F.~Alday, B.~Eden, G.~P.~Korchemsky, J.~Maldacena and E.~Sokatchev,
``From correlation functions to Wilson loops,''
JHEP \textbf{09} (2011), 123
%doi:10.1007/JHEP09(2011)123
[arXiv:1007.3243].

\bibitem{classicalPaper2}
L.~F.~Alday, D.~Gaiotto, J.~Maldacena, A.~Sever and P.~Vieira,
``An Operator Product Expansion for Polygonal null Wilson Loops,''
JHEP \textbf{04} (2011), 088
%doi:10.1007/JHEP04(2011)088
[arXiv:1006.2788].

\bibitem{ourRecentPapers2}
C.~Bercini, V.~Gon\c{c}alves and P.~Vieira,
``Light-Cone Bootstrap of Higher Point Functions and Wilson Loop Duality,''
Phys. Rev. Lett. \textbf{126} (2021) no.12, 121603
%doi:10.1103/PhysRevLett.126.121603
[arXiv:2008.10407].

\bibitem{hexagon4point}
T.~Fleury and S.~Komatsu,
``Hexagonalization of Correlation Functions,''
JHEP \textbf{01}, 130 (2017)
%doi:10.1007/JHEP01(2017)130
[arXiv:1611.05577].

\bibitem{Frank1}
F.~Coronado,
``Perturbative four-point functions in planar $ \mathcal{N}=4 $ SYM from hexagonalization,''
JHEP \textbf{01}, 056 (2019)
%doi:10.1007/JHEP01(2019)056
[arXiv:1811.00467].

\bibitem{Frank2}
F.~Coronado,
``Bootstrapping the Simplest Correlator in Planar $\mathcal N = 4$ Supersymmetric Yang-Mills Theory to All Loops,''
Phys. Rev. Lett. \textbf{124}, no.17, 171601 (2020)
%doi:10.1103/PhysRevLett.124.171601
[arXiv:1811.03282].

\bibitem{DeterminantPapers}
I.~Kostov, V.~B.~Petkova and D.~Serban,
``The Octagon as a Determinant,''
JHEP \textbf{11}, 178 (2019)
%doi:10.1007/JHEP11(2019)178
[arXiv:1905.11467].

\bibitem{nordita}
{See Nordita School on Integrability 2014, Mathematica Notebook by P.Vieira}, \url{https://www.nordita.org/~zarembo/Nordita2014/program.html}

\bibitem{dymasolver}
C.~Marboe and D.~Volin,
``Fast analytic solver of rational Bethe equations,''
J. Phys. A \textbf{50}, no.20, 204002 (2017)
%doi:10.1088/1751-8121/aa6b88
[arXiv:1608.06504].

\bibitem{twist3}
V.~M.~Braun, S.~E.~Derkachov and A.~N.~Manashov,
``Integrability of three particle evolution equations in QCD,''
Phys. Rev. Lett. \textbf{81} (1998), 2020-2023
%doi:10.1103/PhysRevLett.81.2020
[arXiv:hep-ph/9805225]. $\bullet$ V.~M.~Braun, S.~E.~Derkachov, G.~P.~Korchemsky and A.~N.~Manashov,
``Baryon distribution amplitudes in QCD,''
Nucl. Phys. B \textbf{553} (1999), 355-426
%doi:10.1016/S0550-3213(99)00265-5
[arXiv:hep-ph/9902375. $\bullet$ S.~E.~Derkachov, G.~P.~Korchemsky and A.~N.~Manashov,
``Evolution equations for quark gluon distributions in multicolor QCD and open spin chains,''
Nucl. Phys. B \textbf{566} (2000), 203-251
%doi:10.1016/S0550-3213(99)00702-6
[arXiv:hep-ph/9909539].

\bibitem{straight}
One simply use the Baxter equation (\ref{baxterT}) to solve for $\mathbb{Q}^{[+2]}$ in terms of $\mathbb{Q}$ and $\mathbb{Q}^{[-2]}$, plug the result in (\ref{simplifiedBaxter}), use recurrence identities to cancel the Harmonic functions and note that that what is left is zero provided $\mathbb{Q}$ is an even function. This is the case for twist 2 Bethe states.


\bibitem{techremark}
For $\ell_B>1$ the right hand side of (\ref{bernouli2}) is a rational number; the $\pi$'s and the $\zeta(3)$ in the second line are simply cancelling the $\pi$'s and the $\zeta(3)$ generated by the integral. For $\ell_B=1$ the $\pi$'s still cancel but there is no $\zeta(3)$ in the second line. (In that sense the expression is even simpler in this case when wrapping is present!) A $\zeta(3)$ term is generated by the integral so that the rhs of (\ref{bernouli2}) is of the form $\texttt{rational}+\texttt{rational}' \zeta(3)$ as it should.

\bibitem{massage}
In writing (\ref{su2structure}), (\ref{finalgaudin}) we introduced the vacuum integrals $\langle\textbf{1},\textbf{1}\rangle_{\ell,L}$ relative to the naive $\theta$-morphism action in order to simplify the resulting measure and normalizations factors. We also massaged the expression into a manifestly real form. 
%\bibitem{triviality}Non-cyclic non-polynomial-$T$ solutions exist for~$L=2$ at NNLO. 

\bibitem{spintwistsu2}
Note that primary SU(2) operators have $M\geq 2$ and therefore all structure constants for $\ell_{12} = 1$ vanish.

\bibitem{rightbound}
The action of $\partial_{L}$ boundary terms is irrelevant for the non-extremal correlators considered here.

